The many Shapley values for model explanation

The Shapley value has become a popular method to attribute the prediction of a machine-learning model on an input to its base features. The use of the Shapley value is justified by citing [16] showing that it is the \emph{unique} method that satisfies certain good properties (\emph{axioms}). There are, however, a multiplicity of ways in which the Shapley value is operationalized in the attribution problem. These differ in how they reference the model, the training data, and the explanation context. These give very different results, rendering the uniqueness result meaningless. Furthermore, we find that previously proposed approaches can produce counterintuitive attributions in theory and in practice---for instance, they can assign non-zero attributions to features that are not even referenced by the model. In this paper, we use the axiomatic approach to study the differences between some of the many operationalizations of the Shapley value for attribution, and propose a technique called Baseline Shapley (BShap) that is backed by a proper uniqueness result. We also contrast BShap with Integrated Gradients, another extension of Shapley value to the continuous setting.

==> graveyard.tex <==

By a counterfactual input, we mean an input that is contrived for the purpose of generating attributions. For instance, when we apply the Shapley value with the baseline approach (see Section~\ref{sec:baseline}), the contrived inputs stem from intermixing the input and baseline features. For instance, the value of the set function $v(S) = f(x_S;x'_S)$ \checkit{notation}, i.e., some features are drawn from the explicand and others are drawn from the baseline. Even if the explicand and the baseline are natural, this contrived input could be unnatural. Clearly, these contrived inputs could fall outside the training feature distribution, and the model may possibly misbehave on these inputs.
    \footnote{Adversarial examples~\cite{SZSBEGF13} are an instance of such misbehavior. Of course, the adversarial examples are optimized to be adversarial, whereas the contrived inputs are not .} And the model misbehavior could affect the attributions. In this section, we propose an approach that invovles no contrived inputs, i.e., no counterfactuals.
    
\todo{Do I need a concrete example of misbehavior? Can I take imagenet with superpixels and show how the distribution is skewed?}


\section{The Possible Marginals Shapley Value}

The positive of SCE is that when applied on the empirical distribution, it produces attributions without referencing  examples that don't actually occur in the data, this implies that they avoid impossible examples, for instance examples where $Sex=Male$ and $IsMother= True$. The negative of SCE is that the  data distribution can distort the attributions. In this section, we describe a different approach that retains the postives of SCE without its negatives. We call this the Possible Marginals Shapley(PMS) value. 


As in the BS values approach, we have a baseline input $x'$ along with the explicand $x$. As before, the set function $v(S) = f(x_{S}; x'_{N/S})$ \emph{if} the input $x_{S}; x'_{N/S}$ is possible, else we define the $v(S) = \bot$, to denote that the input $x_{S}; x'_{N/S}$ is impossible. We assume that the baseline and the explicand are both possible. 

For instance, suppose you had two features, $Sex$ and $IsMother$. Then the example $Sex=Female,IsMother=False$ is possible whereas the example  $Sex=Male,IsMother=True$ is impossible.

\todo{Impossible worlds can have possible marginals because of the model?}


We define PMS values as a variant of the permutation based definition of Shapley values (cf. Section~\ref{sec:shapley}). The key to the definition is that whenever we construct a set difference in order to perform attribution, the two sets are always valid sets.

\subsection{Examples}

\textbf{Impossible Nearly Everywhere:} In this example, only the explicand the baseline are \emph{possible}. Every other example that is a combination of baseline and explicand features is \emph{impossible}. Here, the attributions to every feature is identical. In this case, we know nothing about the function other than its end-points, and the attributions are "shrunk to the mean". 

\textbf{:} In this example, there are three boolean features $x_1, x_2, x_3$. Examples where $x1=0$ and $x_2=1$ are impossible. Elsewhere, the value of the function $v(x)$ is equal to $x_3$. 


\textbf{:} In this example, there are $n$ boolean features $x_1, x_2, x_3 \ldots x_n$. Examples impossible either when $x1=0$ and $x_2=1$ or when $x1=1$ and $x_2=0$. Elsewhere, the value of the function $v(x)$ is equal to $x_3$. 





\begin{algorithm}
\caption{Possible Marginals Shapley Value}
\begin{algorithmic}
\STATE Input is function $v$.
\STATE \COMMENT{// Compute Shapley values via permutations}
\FORALL{permutations $\sigma$ of $N$}
\STATE $S = \{\}$ \COMMENT{$S$ consists of features that we have visited and successfully added}
\STATE $Z = \{\}$ \COMMENT{$Z$ consists of features that we have visited but not successfully added.}
\STATE \COMMENT{$\sigma_i$ is the $i$th element}
\FORALL{$i \in 1 \ldots |N|$}
\STATE  $Z = Z \cup \sigma_i$.
\IF{$v(S \cup Z) \neq \bot$}
\STATE \COMMENT{Updating Shapley values}
\IF{$|Z| =1$}
\STATE $s_{\sigma_i} \leftarrow s_{\sigma_i} + \frac{v(S \cup Z) - v(S)}{|N|!}$
\ELSE
\STATE $s_{\sigma_i} \leftarrow s_{\sigma_i} + \frac{v(S \cup Z) - v(S)}{2*|N|!}$
\STATE \COMMENT{$z_1$ is the first element added to $Z$}
\STATE $s_{z_1} \leftarrow s_{z_1} + \frac{v(S \cup Z) - v(S)}{2*|N|!}$
\ENDIF
\STATE $Z = \{\}$
\ENDIF
\ENDFOR
\ENDFOR
\end{algorithmic}
\end{algorithm}

We can show that CS values over a set function $v$ are equivalent to BS values over a set function $v'$, that is identical to it at all valid inputs, but is estimated using the set value at subsets of size one less at invalid values.


\begin{algorithm}
\caption{Estimating a marginal $v(S \cup Z) - v(S)$}
\label{alg:est}
\begin{algorithmic}
\STATE \textbf{$Estimate(S,Z)$}
\IF{$v(S) \neq \bot$ and $v(S \cup Z) \neq \bot$}
\STATE return $v(S \cup Z) - v(S)$
\IF{$v(S) = \bot$ and $v(S \cup Z) = \bot$}
\STATE return 0
\IF{$v(S) = \bot$ and $v(S \cup Z) \neq \bot$}
\STATE return $\frac{1}{|S|} \sum_{i \in S} \frac{Estimate(S \setminus i, Z)}{2}$ 
\ELSE
\STATE return $\frac{1}{|N \setminus (Z \cup S)|} \sum_{i \in N \setminus (Z \cup S)} \frac{Estimate(S, Z \cup i)}{2}$
\ENDIF
\ENDIF
\ENDIF
\end{algorithmic}
\end{algorithm}

We assumed that the baseline is valid, so $v(\{\}) \neq \bot$. Therefore if we perform the estimations from the smallest invalid set to the largest, and this results in a consistent definition of $v'$.  

\begin{lemma}
CS Values for a set function $v$ are identical to Shapley values for the set function $v'$ estimated using Algorithm ~\ref{alg:est}. 
\end{lemma}
\begin{proof}


\end{proof}


Here is an example from~\cite{Kahnemann}: A person, who has an ulcer, has eaten some turnips, but forgot to take his medication, and suffers from stomach pain. He attributes it to not having taken the medication, his spouse to his having eaten turnips, and his doctor to the ulcer. All three are possibly valid attributions, but made from three different standpoints; Table~\ref{tab:subj} depicts these standpoints. If $\epsilon, \epsilon_1, \epsilon_2$ all approach zero, then the Shapley value with conditional expectations yields the attributions mentioned above. The interesting thing about the set up is that the doctor and the patient have the same conception of the function; the difference in their attributions stems from the difference in their beliefs about the feature distribution. In contrast, the spouse and the patient have the same feature distribution, but have different conceptions of the function.
 
 
 

\begin{table}[!htb]
    \centering
    \small
    \begin{tabular}{lllllll}
    \hline
     $D_{Doctor}$& $D_{Spouse},D_{Patient}$& Turnip& Ulcer & Medicine & Pain (Doctor/Patient) & Pain(Spouse)\\
     $\epsilon_1 * \epsilon_2$ &  $\epsilon_1 * \epsilon_2$ & \textbf{True} & \textbf{True}& \textbf{False}&\textbf{1} &\textbf{1}\\
     
     $\epsilon_1 * (1- \epsilon_2)$ & $0$ & True & False& False&0 &0\\
     
     $(1-\epsilon_1) * (1-\epsilon_2)$ & $0$ & False & False& False&0 &0\\
     
     $0$ & $\epsilon_1*(1-\epsilon_2)$ & True & True& True&0&1\\
     
     $0$ & $(1-\epsilon_1) *(1-\epsilon_2)$ & False & True& True&0&0\\
     
     $(1-\epsilon_1) * \epsilon_2$ & $(1-\epsilon_1)*\epsilon_2$ & False & True& False&1&0\\
    
    
    \hline
    \hline
    \end{tabular}
    \caption{The doctor and the patient's distributions differ. The spouse and the patient's functions differ.}
    \label{tab:subj}
\vspace{-4mm} %reduce too much white space
\end{table}

\todo{put$T^2B^2$ example back}


In contrast, we have the following theorem:

\begin{theorem}
\label{thm:monotonicity}
Fix an explicand $x$, and distribution $D$ and a feature $i \in Feat(D)$ that is distributed independently from the other features. Given two functions, $f_1$ and $f_2$ such that for all $S \subseteq (N \setminus i)$, the marginal  $f_1(x_{S \cup i};x'_{N\setminus (S \cup i)}) - f_1(x_{S};x'_{N\setminus (S})$ exceeds is at least as large as the marginal $f_2(x_{S \cup i};x'_{N\setminus (S \cup i)}) - f_2(x_{S};x'_{N\setminus (S})$, then the $ces_i(x,D,f_1) \geq ces_i(x,D,f_2)$.
\end{theorem}
\begin{proof}
Fix an explicand $x$ and distribution $D$
satisfying the antecedent of the theorem statement. Recall the expression of the Shapley value (Equation~\ref{eq:shapley}). To complete the proof, we must show that for all sets $S \subseteq (N \setminus i)$, $v(S \cup i) - v(S)$ is larger for function $f_1$ compared to $f_2$, where the set function $v$ is computed using the CES approach (Section~\ref{sec:conditional-expecations}).

For a some function $f \in \{f1,f2\}$: 

\begin{equation}
\label{eq1}
v(S) = \sum_{S \subseteq T \subseteq N} f(x_T; x'_{N/T}) \prod_{j \in T \setminus S} p_j * \prod_{j \in N \setminus T} p_j
\end{equation}

Similarly: 

\begin{equation}
\label{eq2}
v(S \cup i) = \sum_{S \cup i \subseteq T \subseteq N} f(x_T; x'_{N/T}) \prod_{j \in T \setminus (S \cup i)} p_j * \prod_{j \in N \setminus T} p_j    
\end{equation}

Equation~\ref{eq1} can be be rewritten as to match the number of terms in Equation~\ref{eq2}:

\begin{equation}
\label{eq3}
v(S) = \sum_{S \cup i \subseteq T \subseteq N} \prod_{j \in T \setminus (S \cup i)} p_j * \prod_{j \in N \setminus T} p_j \left(p_i * f(x_T; x'_{N/T}) + (1-p_i) * f(x_{T \setminus i}; x'_{N \setminus (T \setminus i)}) \right)
\end{equation}

Subtracting, Equation~\ref{eq3} from Equation~\ref{eq2} we get: 
\begin{equation}
\label{eq4}
v(S \cup i) - v(S) = \sum_{S \cup i \subseteq T \subseteq N} \prod_{j \in T \setminus (S \cup i)} p_j * \prod_{j \in N \setminus T} p_j * (1-p_i) * \left(f(x_T; x'_{N/T}) - f(x_{T \setminus i}; x'_{N \setminus (T \setminus i)}) \right)
\end{equation}

This equation is monotone in the marginals 
$f(x_{S \cup i};x'_{N\setminus (S \cup i)}) - f(x_{S};x'_{N\setminus (S})$, proving the result.
\end{proof}

\section{Explore and Explain}
\todo{add a remark about IG and realism}

Thus far, we have discussed two extremes for distributions in the context of attribution by conditional expectation --- on the one extreme, D is precisely the empirical distribution while on the other D is implied (revealed) by a given explanation (set of attributions). \checkit{I think the other extreme is a posited distribution, which is not necessarily revealed. Take, for instance, the baseline approach or the Datta approach. The distribution is explicitly posited, but I don't think it changes your point.} The former (NCS) is entirely realistic with respect to the data, but may result in counterintuitive attributions. In particular, NCS does not generalize beyond the strict set of observations and hence fails (gives trivial attributions) when there is any data sparsity. On the other extreme, the revealed distribution is used to justify a given explanation (set of attributions) and therefore cannot result in unexpected attributions. \checkit{I'd say the reason the attributions are not counterintuitive is because the distribution has separability or some other condition.} But being entirely subordinate to the attribution procedure, the revealed distribution makes no attempt at realism whatsoever. In either case there may be discomfort --- either from counterintuitive attributions or from the unrealistic counterfactuals implied by the revealed distribution. Between these extremes are approaches which make compromises between realism and the intuitiveness of attribution. We explore some of these approaches. In what follows, we mention connections to causal inference in statistics wherein appropriate.

\subsection{Estimating a distribution}
An obvious failure of NCS is that it does not generalize beyond the given observations.  \checkit{what do you think about trees here? we can discuss.}

One particular approach to density estimation is to assume independence among the features. Marginal distributions are easier to estimate and, for discrete features, may not suffer from any data sparsity. In this case, each marginal is estimated separately and the joint distribution is assumed to be the product of marginals. We have already described the implications of independent feature distributions for conditional expectation attribution --- loosely-speaking, they are more intuitive. But we should draw a clear distinction between the reasons for assuming an independent feature distribution. Are we doing this to overcome the curse of dimensionality in density estimation, or to produce more intuitive attributions? This is not always clear in the literature (e.g. \cite{Datta}). If enforcing independence of the sake of intuitive attributions is the goal, then why necessarily restrict ourselves to the empirical marginal distribution of features? \checkit{(Frankenstein posited) Let us discuss this.}.

In either case, we face potential discomfort from lack of realism due to the mismatch between the empirical distribution and assumed independent distribution. In high dimensional space, there are bound to be regions with no observations to which we assign non-zero probability. But even in the low-dimensional, discrete setting where we may have observations in every cell, there are challenges. Expectations over the independent distribution can be thought of as expectations over individual observations with weights such that the reweighted empirical distribution matches the independent distribution (footnote: reweighting by propensity score does essentially this, but only for the one binary treatment variable whose causal effect is to be estimated). It may be the case that certain cells with few observations may require very large weights and hence have disproportionate impact on the explanation. We may ask ourselves whether there is something categorically different about these rare observations. \checkit{example??? height/weight in humans, true example of black Trump supporter, omitted variable bias, outliers, unicorns?)}

\subsection{Experimentation}
\checkit{I think we have to say something about the case where the function is treated as a given (either because it is the deployed model, or because it is authored) versus when it is learned and the phenomena is the real thing.}

Lack of observations in density estimation can be remedied most directly by collecting additional observations. When this is feasible, it can help with the explanation because the function is evaluated only with real observations. Indeed, if the data is not given and must be collected, one may benefit from putting thought into how the data is collected. This is the area of Design Of Experiments in statistics [Fisher, 1935]. Statisticians have long been aware that orthogonality in the feature space results in better estimation due to balance. However, unlike the current treatment, their concern was largely to fit and interpret linear models, most notably the causal effect of differing treatments. We should note that the effort to ensure orthogonality in the data collection may itself be subject to the criticism of lack of realism. For example, to separate the causal effects of soil from rainfall may require the experimenter to vary both independently, even though soil and rainfall might not vary independently in nature. \checkit{(Frankenstein realized)}.

\subsection{Restricting scope of the explanation}
In some cases, we may be unwilling to generalize beyond the observations to the point of independence. For instance, we may be unwilling to rely heavily on the rare observations in certain cells, let alone posit that they exist without having seen them. In such cases, it might make sense to limit the scope of the explanation. This happens often in the context of causal inference from observation. For instance, if we lack the data, or credulity to extrapolate a model to affluent mothers of crack babies, we cannot fully separate the effects of socioeconomic status from the use of crack. Instead, we may simply restrict our causal inference to the effects of crack on mothers from low SES. We can do likewise for attribution of models. In cases where the independent feature distribution across the whole space is implausible, we may restrict the explanation to a region of the space where the independent feature distribution is more tenable. \checkit{We need an example here perhaps.}

\subsection{Reabstraction}
One final approach to dealing with an implausible independent feature distribution is to change the features themselves. In certain cases, an independent distribution is more plausible for a transform of the original features. For example, instead of height, weight and age for adult males we might have a more plausible independent distribution of BMI and age. The resulting explanation of the function will be in terms of BMI and age, even though the function may use height, weight and age. The success of an approach rests on the intuitiveness of the transformed features and may be preferable to imagining or observing adult males measuring 6 ft 3 in height and 100 lb. \checkit{nice example!}

\subsection{Summary}
It may sound impossible to square the requirements of an intuitive attribution method with the limitations of any finite set of observations, however collected. \checkit{is it finiteness or unbreakable correlations?} The point we wish to make here is that this is what humans do all the time. They may do this with varying levels of awareness and sophistication, everywhere from mundane situations to scientific investigations. The purpose of this paper is (1) to elaborate the assumptions underlying various approaches to attribution, each of which may be cast as making assumptions about the feature distribution, and (2) to describe how the limits of observation can nevertheless transcended by judgment.

\section{Proofs}








In contrast, we have the following theorem:
\begin{theorem}
\label{thm:dummy}
Fix a function $f$, a distribution $D$ and an explicand $x$. Consider a feature $i \in \Feat(D)$ but not in $\Feat(f)$ that is independently distributed from all the features in $\Feat(F)$. Then $ces_i(x, D,f)$ is zero. 
\end{theorem}

We first prove a technical lemma that we will use to prove this theorem and reuse later. 

\begin{lemma}[Deletion Lemma]
Given a function $f$, a distribution $D$, an explicand $x$, if the features in $\Feat(f)$ are independent from some features in $G \subseteq \Feat(D) \setminus \Feat(f)$, then for all sets $S \subseteq \Feat(D)$, the conditional expectation $E[f(x)|x_S]$ is equal to the conditional expectation that marginalizes over features in $G$, i.e, $E[f(x)|x_{S \setminus G}]$.
\end{lemma}
\begin{proof}

\begin{eqnarray*}
E[f(x)|x_S] 
&=& \sum_{x'|x'_S = x_S} f(x')* \frac{P[x']}{P[x'_S = x_S]}\\
&=& \sum_{x'|x'_S = x_S} f(x')* \frac{P[x'_{\Feat(f)}] * P[x'_{G}]}{P[x'_{S\cap \Feat(f)} = x_{S\cap \Feat(f)} ] * P[x'_{S\cap G} = x_{S\cap G}]}\\
&=& \sum_{x'|x'_S = x_S} f(x'_\Feat(f))* \frac{P[x'_{\Feat(f)}] * P[x'_{G}]}{P[x'_{S\cap \Feat(f)} = x_{S\cap \Feat(f)} ] * P[x'_{S\cap G} = x_{S\cap G}]}\\
&=& \sum_{x'_{\Feat(f)}|x'_{S \cap \Feat(f)} = x_{S cap \Feat(f)}} f(x'_\Feat(f))* \frac{P[x'_{\Feat(f)}]}{P[x'_{S\cap \Feat(f)}]} * \sum_{x'_{G}|x'_{S \cap G} = x_{S \cap G}} \frac{P[x'_{G}]}{P[x'_{S\cap G}]} \\
&=& \sum_{x'_{\Feat(f)}|x'_{S \cap \Feat(f)} = x_{S \cap \Feat(f)}} f(x'_\Feat(f))* \frac{P[x'_{\Feat(f)}]}{P[x'_{S\cap \Feat(f)}]}\\
&=& E[f(x)|x_{S \setminus G}]
\end{eqnarray*}

The first and last steps are by definition of the conditional expectation, the second step is because features $\Feat(f)$ are independent from those in $G$, the third step is because $f$ is insensitive to features in $G$, and the fourth step is 
by breaking the choice of $x'$ into two choices, those of the features in $F$ and those of features in $G$, the fifth step is by marginalizing over features in $G$. 
\end{proof}

\begin{proof} [Proof of Theorem~\ref{thm:dummy}]
Recall the formula for the Shapley value(\ref{eq:shapley}). To complete the proof, we show that the value of  $E[f(x')| x'_{\Feat(S \cup i)} = x_{\Feat(S \cup i)}] -  E[f(x')| x'_{\Feat(S_j)} = x_{\Feat(S_j)}]$ is zero for all sets $S \subseteq D$. This is true because of the Deletion lemma with the singleton set $\{i\}$ playing the role of set $G$.  
\end{proof}

\subsubsection{The Additivity Axiom}
\label{sec:add}

\todo{mention stuff about an ensemble of trees}

.




\todo{turn theorems into remark}

We now have the following lemma:  

\begin{theorem}
\label{thm:additivity}
For every two functions $f_1$ and $f_2$, a feature distribution $D$ over every feature in $\Feat(D_1) \cup \Feat(D_2)$, every feature $i \in \Feat(D_1) \cup \Feat(D_2)$ and every explicand $x$ that specifies values for all the variables in $\Feat(D_1) \cup \Feat(D_2)$: 
If (a) If unreferenced variables have zero attributions, i.e., for all $j \notin \Feat(D)$, $ces_j(x,D,f) = 0$.
(b) If for all $j \notin \Feat(D_1)$, $j$ is distributed independently (in $D$) of all the features in $\Feat(D_1)$.
(c) If for all $j \notin \Feat(D_2)$, $j$ is distributed independently (in $D$) of all the features in $\Feat(D_2)$.
then, $ces_j(x,D,f_1 + f_2) =
ces_j(x_{\Feat(D_1)},D_1,f_1) + ces_j(x_{\Feat(D_2)},D_2,f_2)$; here $D_1$ and $D_2$ marginalize the distribution $D$ over all the features not in $\Feat(D_1)$ and $\Feat(D_1)$ respectively.
\end{theorem}
\begin{proof}
Fix two functions $f_1$ and $f_2$ and a feature $j$. We do the proof in two steps. We first show that $ces_j(x,D,f_1 + f_2) = ces_j(x_{\Feat(D_1)},D,f_1) + ces_j(x_{\Feat(D_2)},D,f_2)$. Second, we show that $ces_j(x_{\Feat(D_1)},D,f_1) = ces_j(x_{\Feat(D_1)},D_1,f_1)$ (and symmetrically, $ces_j(x_{\Feat(D_2)},D,f_2) = ces_j(x_{\Feat(D_2)},D,f_2)$). This completes the proof. 

 Notice that the formula for the Shapley value (Equation~\ref{eq:shapley}) is linear in the set function values $v(S)$, for all $S \subseteq N$. By the definition of CES (Section~\ref{sec:conditional-expecations}, it is sufficient to show that
 $E[f_1(x_{\Feat(D_1)}) + f_2(x_{\Feat(D_2)})|x_S)] = E_D[f(x_{\Feat(D_1)})|x_S)] + E_D[f(x_{\Feat(D_2)})|x_S)]$. But this is true by linearity of expectations. This completes the first step.
 
 
 Next, we show that $ces_j(x_{\Feat(D_1)},D,f_1) = ces_j(x_{\Feat(D_1)},D_1,f_1)$. There are two cases. If $j \notin \Feat(D_1)$, the RHS is zero by assumption, and the LHS is zero by Lemma~\ref{thm:dummy}, because $j$ is independently distributed from features in $\Feat(D_1)$.  
  
 On the other hand, if $j \in \Feat(D_1)$, we need to show that marginalizing over variables outside $\Feat(D_1)$ does not change its CES attribution. Let us compute the Shapley value using the permutation based approach. Fix a permutation $\sigma$  over all the features of $\Feat(D_1)$. Let $S_j \subseteq \Feat(D_1)$ consist of all the features that precede $j$ in $\sigma$.
 The attribution to $j$ from this permutation is:
 \begin{equation}
 \label{exp:marginal}
 E[f(x'_{\Feat(D_1)})| x'_{\Feat(S_j \cup i)} = x_{\Feat(S_j \cup i)}] - E[f(x'_{\Feat(D_1)})| x'_{\Feat(S_j)} = x_{\Feat(S_j)}]
  \end{equation}
 
And the weight of this permutation is $1/(\Feat(D_1)!$. Now consider the permutations over the features of $\Feat(D)$ consistent with the permutation $\sigma$. 
The attribution to $j$ from every one of these permutations is identical to that in Expression~\ref{exp:marginal}: Suppose $S'_j \subseteq D$ is the set of features that precede $j$ in one of these permutations, then $E[f(x'_{\Feat(D)})| x'_{\Feat(S'_j \cup j)}$ is the same as $E[f(x'_{\Feat(D_1)})| x'_{\Feat(S_j \cup j)}$ and $E[f(x'_{\Feat(D)})| x'_{\Feat(S'_j )}$ is the same as $E[f(x'_{\Feat(D_1)})| x'_{\Feat(S_j)}$ by two applications of the Deletion Lemma with $S'_j - S_j$ playing the role of $G$.

Each permutation has a weight of $1/(\Feat(D)!$ and there are a total of $(\Feat(D)!/(\Feat(D_1)!$ such permutations; thus their cumulative weight is the same as that in the calculation with just the features in $\Feat(D_1)$. This completes the proof.
\end{proof}



\begin{theorem}
\label{thm:symmetry}
If two variables are distributed identically, if they have identical values in the explicand, and if they are symmetric in the function, then their attributions are equal.
\end{theorem}
\begin{proof}
Sketch: The CES computation for variable $i$ and $j$ are identical. 
\end{proof}
